Automata-Theoretic Verification of Interval Markov Decision Processes

Interval Markov decision processes (IMDPs) provide a natural framework for modeling stochastic systems with uncertain transition probabilities, represented by probability intervals and resolved adversarially. Such uncertainty arises naturally, for example, when the transition model is learned from finite data or obtained through model-based reinforcement learning. In this paper, we study the automata-theoretic verification of IMDPs against rich temporal specifications, including all LTL specifications, by considering the broader class of {\omega}-regular objectives. We show that classical automata-theoretic verification techniques extend to IMDPs, but with a sharp distinction determined by the structure of the transition intervals. For stable IMDPs, where either the upper bound is zero or the lower bound is strictly positive, verification reduces to ordinary MDP analysis and can be carried out using the standard automata used in that setting (good-for-MDP automata). For unstable IMDPs, where intervals may include zero while the upper bound is strictly positive, verification becomes game-like and requires automata whose nondeterminism can be resolved on the fly (good-for-games automata). Building on these insights, we develop algorithms for verifying {\omega}-regular specifications over IMDPs and derive probabilistic guarantees when the interval model is learned from sampled data. The resulting framework enables principled verification of stochastic systems under probabilistic model uncertainty, connecting automata-based verification with data-driven stochastic modeling.

==> Figures/experiments_table_automata1.tex <==


% \begin{scriptsize}
% \begin{center}
% \begin{tabular}{|c|c|c|c|c|c|c|}
% \hline

% \multirow{3}{*}{\textbf{Model}} 
%   & \multicolumn{2}{c|}{\textbf{IMDP Properties}} 
%   & \multicolumn{2}{c|}{\textbf{algorithms timing (sec)}} 
%   & \multirow{3}{*}{\textbf{VI Iterations}} 
%   & \multirow{3}{*}{\makecell{\textbf{Qualitative} \\ \textbf{time}}}
% \\ \cline{2-5}

% & \makecell{\textbf{number of} \\ \textbf{States}}
% & \makecell{\textbf{million} \\ \textbf{Transitions}}
% & \textbf{Policy Iteration}
%  & \textbf{Value Iteration} 
%  & 
%  & 
% \\
% \hline
% \hline

% \multirow{8}{*}{\textbf{UAV}} 
%  & 784  & 0.5  & 68.54  & 31.49  & 16 & 1.12 \\ 
%  & 1024 & 1    & 133.23 & 50.75  & 12 & 1.53 \\ 
%  & 1296 & 2    & 310.01 & 154.14 & 19 & 2.88 \\ 
%  & 1600 & 3    & 483.56 & 233.79 & 17 & 4.34 \\ 
%  & 1800 & 5    & 1007.98 & 655.54 & 21 & 8.39 \\ 
%  & 2160 & 9    & 3356.64 & 2068.86 & 25 & 145.14 \\ 
%  & 2304 & 12   & 4066.91  & 3207.98 & 30 & 163.57 \\ 
%  & 2430 & 15   & 6351.37 & 7973.71 & 41 & 274.74 \\
 
% \hline
% \hline

% \multirow{3}{*}{\textbf{Shuttle}} 
%  & 3200 & 1  & 133.50 & 41.35 & 6 & 6.97 \\ 
%  & 5000 &  2 & 504.84 & 106.06 & 6 & 18.08 \\ 
%  & 7200 &  6 & 2188.25  & 316.55 & 6 & 59.01 \\
% \hline

% \end{tabular}
% \end{center}
% \end{scriptsize}







% \begin{scriptsize}
% \begin{center}
% \begin{tabular}{l|cc|cc|c|c}

% \toprule
% \multirow{3}{*}{\textbf{Model}} 
% & \multicolumn{2}{c|}{\textbf{IMDP properties}}
% & \multicolumn{2}{c|}{\textbf{Algorithms timing (sec)}}
% & \multirow{3}{*}{\makecell{\textbf{Value Iteration} \\ \textbf{counts}}}
% & \multirow{3}{*}{\makecell{\textbf{Qualitative} \\ \textbf{time (sec)}}}
% \\
% \cmidrule(lr){2-3} \cmidrule(lr){4-5}
% & \makecell{\textbf{number of} \\ \textbf{states}} 
% & \makecell{\textbf{million} \\ \textbf{transitions}}
% & \makecell{\textbf{Policy} \\ \textbf{Iteration}}
% & \makecell{\textbf{Value} \\ \textbf{Iteration}}
% & & 
% \\
% \midrule

% \multirow{8}{*}{\textbf{UAV} }
%  & 784  & 0.5  & 68.54  & 31.49  & 16 & 1.12 \\ 
%  & 1024 & 1    & 133.23 & 50.75  & 12 & 1.53 \\ 
%  & 1296 & 2    & 310.01 & 154.14 & 19 & 2.88 \\ 
%  & 1600 & 3    & 483.56 & 233.79 & 17 & 4.34 \\ 
%  & 1800 & 5    & 1007.98 & 655.54 & 21 & 8.39 \\ 
%  & 2160 & 9    & 3356.64 & 2068.86 & 25 & 145.14 \\ 
%  & 2304 & 12   & 4066.91  & 3207.98 & 30 & 163.57 \\ 
%  & 2430 & 15   & 6351.37 & 7973.71 & 41 & 274.74 \\
% \midrule
% \multirow{3}{*}{\textbf{Shuttle}} 
%  & 3200 & 1  & 133.50 & 41.35 & 6 & 6.97 \\ 
%  & 5000 & 2 & 504.84 & 106.06 & 6 & 18.08 \\ 
%  & 7200 & 6 & 2188.25  & 316.55 & 6 & 59.01 \\
% \bottomrule

% \end{tabular}
% \end{center}
% \end{scriptsize}


\begin{table}[t]
\caption{Performance results on SIMDP benchmarks for $(\mathbf{F}\mathit{reach} \land \mathbf{G}\neg\mathit{deadlock})$: size, value iteration (VI) and strategy improvement (SI)
runtimes, and qualitative reachability solving time.}
\vspace{1.5mm}
\label{tab:exp-results-automata1}
\centering
\scriptsize
\setlength{\tabcolsep}{6pt}
\begin{tabular}{l|cc|cc|rc|c}
\toprule
\multirow{3}{*}{\textbf{Model}} 
& \multicolumn{2}{c|}{\textbf{SIMDP size}}
& \multicolumn{2}{c|}{\textbf{runtime (sec)}} 
& \multicolumn{2}{c|}{\textbf{iterations count}} 
% & \multirow{3}{*}{\textbf{SI iters}}
% & \multirow{3}{*}{\textbf{VI iters}}
& \multirow{3}{*}{\textbf{Qual.\ time}} 
\\
\cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}
& \textbf{states}
& \makecell{\textbf{transitions}\\(\textbf{millions})}
& \textbf{SI}
& \textbf{VI}
& \textbf{SI}
& \textbf{VI}
& \\
\midrule

\multirow{8}{*}{\textbf{UAV}}
 & 784  & 0.5  & 68.54   & 31.49   & 4 & 16 & 1.12 \\
 & 1024 & 1    & 133.23  & 50.75   & 4 & 12 & 1.53 \\
 & 1296 & 2    & 310.01  & 154.14  & 4 & 19 & 2.88 \\
 & 1600 & 3    & 483.56  & 233.79  & 4 & 17 & 4.34 \\
 & 1800 & 5    & 1007.98 & 655.54  & 4 & 21 & 8.39 \\
 & 2160 & 9    & 3356.64 & 2068.86 & 6 & 25 & 145.14 \\
 & 2304 & 12   & 4066.91 & 3207.98 & 6 & 30 & 163.57 \\
 & 2430 & 15   & 6351.37 & 7973.71 & 6 & 41 & 274.74 \\
\midrule

\multirow{3}{*}{\textbf{Shuttle}}
 & 3200 & 1 & 133.50 & 41.35 & 3 & 6 & 6.97 \\
 & 5000 & 2 & 504.84 & 106.06 & 3 & 6 & 18.08 \\
 & 7200 & 6 & 2188.25 & 316.55 & 3 & 6 & 59.01 \\
\bottomrule
\end{tabular}
\vspace{-4.5mm}
\end{table}


==> Figures/expre_res_3_gr1_plots.tex <==

\begin{figure*}[h]
    \centering    
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \includegraphics[width=\linewidth]{Figures/gr1_uav_si_time_vs_transitions.png}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \includegraphics[width=\linewidth]{Figures/gr1_uav_vi_time_vs_transitions.png}
    \end{subfigure}
    \hfill
        \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \includegraphics[width=\linewidth]{Figures/gr1_uav_qual_time_vs_transitions.png}
    \end{subfigure}
    \caption{
Performance comparison for the UAV benchmarks under the GR(1) specifications as a function of the number of transitions. Each plot corresponds to Strategy Improvement (left), Value Iteration (middle), and Qualitative Analysis (right). Times are reported in seconds. The legend is shown only once; the same color-to-specification mapping holds for all plots.
    }
    \label{fig:gr1_uav_results}
\end{figure*}


==> Figures/initial_states/experiments_table.tex <==


% \begin{scriptsize}
% \begin{center}
% \begin{tabular}{|c|c|c|c|c|c|c|}
% \hline

% \multirow{3}{*}{\textbf{Model}} 
%   & \multicolumn{2}{c|}{\textbf{IMDP Properties}} 
%   & \multicolumn{2}{c|}{\textbf{algorithms timing (sec)}} 
%   & \multirow{3}{*}{\textbf{VI Iterations}} 
%   & \multirow{3}{*}{\makecell{\textbf{Qualitative} \\ \textbf{time}}}
% \\ \cline{2-5}

% & \makecell{\textbf{number of} \\ \textbf{States}}
% & \makecell{\textbf{million} \\ \textbf{Transitions}}
% & \textbf{Policy Iteration}
%  & \textbf{Value Iteration} 
%  & 
%  & 
% \\
% \hline
% \hline

% \multirow{8}{*}{\textbf{UAV}} 
%  & 784  & 0.5  & 68.54  & 31.49  & 16 & 1.12 \\ 
%  & 1024 & 1    & 133.23 & 50.75  & 12 & 1.53 \\ 
%  & 1296 & 2    & 310.01 & 154.14 & 19 & 2.88 \\ 
%  & 1600 & 3    & 483.56 & 233.79 & 17 & 4.34 \\ 
%  & 1800 & 5    & 1007.98 & 655.54 & 21 & 8.39 \\ 
%  & 2160 & 9    & 3356.64 & 2068.86 & 25 & 145.14 \\ 
%  & 2304 & 12   & 4066.91  & 3207.98 & 30 & 163.57 \\ 
%  & 2430 & 15   & 6351.37 & 7973.71 & 41 & 274.74 \\
 
% \hline
% \hline

% \multirow{3}{*}{\textbf{Shuttle}} 
%  & 3200 & 1  & 133.50 & 41.35 & 6 & 6.97 \\ 
%  & 5000 &  2 & 504.84 & 106.06 & 6 & 18.08 \\ 
%  & 7200 &  6 & 2188.25  & 316.55 & 6 & 59.01 \\
% \hline

% \end{tabular}
% \end{center}
% \end{scriptsize}







% \begin{scriptsize}
% \begin{center}
% \begin{tabular}{l|cc|cc|c|c}

% \toprule
% \multirow{3}{*}{\textbf{Model}} 
% & \multicolumn{2}{c|}{\textbf{IMDP properties}}
% & \multicolumn{2}{c|}{\textbf{Algorithms timing (sec)}}
% & \multirow{3}{*}{\makecell{\textbf{Value Iteration} \\ \textbf{counts}}}
% & \multirow{3}{*}{\makecell{\textbf{Qualitative} \\ \textbf{time (sec)}}}
% \\
% \cmidrule(lr){2-3} \cmidrule(lr){4-5}
% & \makecell{\textbf{number of} \\ \textbf{states}} 
% & \makecell{\textbf{million} \\ \textbf{transitions}}
% & \makecell{\textbf{Policy} \\ \textbf{Iteration}}
% & \makecell{\textbf{Value} \\ \textbf{Iteration}}
% & & 
% \\
% \midrule

% \multirow{8}{*}{\textbf{UAV} }
%  & 784  & 0.5  & 68.54  & 31.49  & 16 & 1.12 \\ 
%  & 1024 & 1    & 133.23 & 50.75  & 12 & 1.53 \\ 
%  & 1296 & 2    & 310.01 & 154.14 & 19 & 2.88 \\ 
%  & 1600 & 3    & 483.56 & 233.79 & 17 & 4.34 \\ 
%  & 1800 & 5    & 1007.98 & 655.54 & 21 & 8.39 \\ 
%  & 2160 & 9    & 3356.64 & 2068.86 & 25 & 145.14 \\ 
%  & 2304 & 12   & 4066.91  & 3207.98 & 30 & 163.57 \\ 
%  & 2430 & 15   & 6351.37 & 7973.71 & 41 & 274.74 \\
% \midrule
% \multirow{3}{*}{\textbf{Shuttle}} 
%  & 3200 & 1  & 133.50 & 41.35 & 6 & 6.97 \\ 
%  & 5000 & 2 & 504.84 & 106.06 & 6 & 18.08 \\ 
%  & 7200 & 6 & 2188.25  & 316.55 & 6 & 59.01 \\
% \bottomrule

% \end{tabular}
% \end{center}
% \end{scriptsize}


\begin{table}[t]
\caption{Performance results on SIMDP benchmarks: size, value iteration (VI) and strategy iteration (SI)
runtimes, and qualitative reachability solving time.}
\vspace{1.5mm}
\label{tab:exp-results}
\centering
\scriptsize
\setlength{\tabcolsep}{6pt}
\begin{tabular}{l|cc|cc|rc|c}
\toprule
\multirow{3}{*}{\textbf{Model}} 
& \multicolumn{2}{c|}{\textbf{SIMDP size}}
& \multicolumn{2}{c|}{\textbf{runtime (sec)}} 
& \multicolumn{2}{c|}{\textbf{iterations count}} 
% & \multirow{3}{*}{\textbf{SI iters}}
% & \multirow{3}{*}{\textbf{VI iters}}
& \multirow{3}{*}{\textbf{Qual.\ time}} 
\\
\cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}
& \textbf{states}
& \makecell{\textbf{transitions}\\(\textbf{millions})}
& \textbf{SI}
& \textbf{VI}
& \textbf{SI}
& \textbf{VI}
& \\
\midrule

\multirow{8}{*}{\textbf{UAV}}
 & 784  & 0.5  & 68.54   & 31.49   & 4 & 16 & 1.12 \\
 & 1024 & 1    & 133.23  & 50.75   & 4 & 12 & 1.53 \\
 & 1296 & 2    & 310.01  & 154.14  & 4 & 19 & 2.88 \\
 & 1600 & 3    & 483.56  & 233.79  & 4 & 17 & 4.34 \\
 & 1800 & 5    & 1007.98 & 655.54  & 4 & 21 & 8.39 \\
 & 2160 & 9    & 3356.64 & 2068.86 & 6 & 25 & 145.14 \\
 & 2304 & 12   & 4066.91 & 3207.98 & 6 & 30 & 163.57 \\
 & 2430 & 15   & 6351.37 & 7973.71 & 6 & 41 & 274.74 \\
\midrule

\multirow{3}{*}{\textbf{Shuttle}}
 & 3200 & 1 & 133.50 & 41.35 & 3 & 6 & 6.97 \\
 & 5000 & 2 & 504.84 & 106.06 & 3 & 6 & 18.08 \\
 & 7200 & 6 & 2188.25 & 316.55 & 3 & 6 & 59.01 \\
\bottomrule
\end{tabular}
\vspace{-4.5mm}
\end{table}

